Nonlinear computations in spiking neural networks through multiplicative synapses

The brain efficiently performs nonlinear computations through its intricate networks of spiking neurons, but how this is done remains elusive. While nonlinear computations can be implemented successfully in spiking neural networks, this requires supervised training and the resulting connectivity can be hard to interpret. In contrast, the required connectivity for any computation in the form of a linear dynamical system can be directly derived and understood with the spike coding network (SCN) framework. These networks also have biologically realistic activity patterns and are highly robust to cell death. Here we extend the SCN framework to directly implement any polynomial dynamical system, without the need for training. This results in networks requiring a mix of synapse types (fast, slow, and multiplicative), which we term multiplicative spike coding networks (mSCNs). Using mSCNs, we demonstrate how to directly derive the required connectivity for several nonlinear dynamical systems. We also show how to carry out higher-order polynomials with coupled networks that use only pair-wise multiplicative synapses, and provide expected numbers of connections for each synapse type. Overall, our work demonstrates a novel method for implementing nonlinear computations in spiking neural networks, while keeping the attractive features of standard SCNs (robustness, realistic activity patterns, and interpretable connectivity). Finally, we discuss the biological plausibility of our approach, and how the high accuracy and robustness of the approach may be of interest for neuromorphic computing.

==> preambule.tex <==
%%%%%%%%%%TO FORMAT A PREPRINT%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage[top=7cm,bottom=2.5cm,headheight=120pt,headsep=15pt,left=6cm,right=1.5cm,marginparwidth=4.2cm,marginparsep=0.5cm]{geometry}


\usepackage{marginnote}
\reversemarginpar  % sets margin notes to the left
\usepackage{lipsum} % Required to insert dummy text
\usepackage{calc}
\usepackage{siunitx}
\usepackage{lineno}
%\usepackage[none]{hyphenat} % use only if there is a problem
% Use Unicode characters
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
% Clean citations with biblatex
\usepackage[
backend=biber,
natbib=true,
sortcites=true,
defernumbers=true,
style=authoryear,
citestyle=authoryear-comp,
maxnames=99,
maxcitenames=2,
giveninits=true,
terseinits=true,
url=false
]{biblatex}
\DeclareNameAlias{default}{family-given}
\renewcommand*{\revsdnamepunct}{} % no comma between family and given names
\renewbibmacro{in:}{%
  \ifentrytype{article}{}{\printtext{\bibstring{in}\intitlepunct}}} % remove 'In:' before journal name
\DeclareFieldFormat[article]{pages}{#1} % remove pp.
\AtEveryBibitem{\ifentrytype{article}{\clearfield{number}}{}} % don't print issue numbers
\DeclareFieldFormat[article, inbook, incollection, inproceedings, misc, thesis, unpublished]{title}{#1} % title without quotes
\usepackage{csquotes}
\RequirePackage[english]{babel} % must be called after biblatex
\addbibresource{sample.bib}
\DeclareBibliographyCategory{ignore}
\addtocategory{ignore}{recommendation} % adding recommendation to 'ignore' category so that it does not appear in the References
% Clickable references. Use \url{www.example.com} or \href{www.example.com}{description} to add a clicky url
\usepackage{nameref}
\usepackage[pdfborder={0 0 0}]{hyperref}  % sets link border to white
\urlstyle{same}

\if{\PCI=cneuro}{\newcommand{\logo}{logo_pour_PDF_evolbiol.png}}\fi


%logo_pour_PDF_cneuro.png
%small_logo_pour_PDF_cneuro.png
%Peer Community In Circuit Neuroscience


% Include figures
\usepackage{graphbox}  % loads graphicx ppackage with extended options for vertical alignment of figures
% Line numbers
%\usepackage[right]{lineno}
% Improve typesetting in LaTex
\usepackage{microtype}
\DisableLigatures[f]{encoding = *, family = * }
% Text layout and font (Open Sans)
\setlength{\parindent}{0.4cm}
\linespread{1.2}
\RequirePackage[default,scale=0.90]{opensans}
% Defining document colors
\usepackage{xcolor}
\definecolor{darkgray}{HTML}{808080}
\definecolor{mediumgray}{HTML}{6D6E70}
\definecolor{ligthgray}{HTML}{d9d9d9}
\definecolor{pciblue}{HTML}{74adca}
\definecolor{opengreen}{HTML}{77933c}
% Use adjustwidth environment to exceed text width
\usepackage{changepage}
% Adjust caption style
\usepackage[aboveskip=1pt,labelfont=bf,labelsep=period,singlelinecheck=off]{caption}

% Headers and footers
\usepackage{fancyhdr}  % custom headers/footers
\usepackage{lastpage}  % number of page in the document
\pagestyle{fancy}  % enables customization of headers/footers
\fancyhfoffset[L]{4.5cm}  % offsets header and footer to the left to include margin
\renewcommand{\headrulewidth}{\ifnum\thepage=1 0.5pt \else 0pt \fi} % header ruler only on first page
\renewcommand{\footrulewidth}{0.5pt}
% full logo on first page, then small logo on subsequent pages 

\lhead{\ifnum\thepage=1 \includegraphics[width=13.5cm]{\logo} \else \includegraphics[width=5cm]{small_logo_pour_PDF_cneuro.png} \fi}  

\chead{}
\rhead{}

\newcommand{\DOIlink}{\href{https://dx.doi.org/\DOI}{\DOI}}

\newcommand{\DOIrecommendationlink}{\href{https://dx.doi.org/\DOIrecommendation}{\DOIrecommendation}}

\lfoot{\scriptsize \textsc{\color{mediumgray}\PCI}}

\cfoot{}
\rfoot{\scriptsize\thepage\space of\space\pageref{LastPage}}


\newcommand{\PCI}{Peer Community In Circuit Neuroscience}


\newcommand{\beginingpreprint}{
\vspace*{0.5cm}
\begin{flushleft}
\baselineskip=30pt
%\marginpar{\includegraphics[align=c,width=0.5cm]{OAlogogreen.png} \space %\large\textbf{\color{opengreen}Open Access}\\
%\\
%\large\textnormal{\color{opengreen}PREPRINT}}
% Margin information
\marginpar{
\large\textnormal{\color{pciblue}\\RESEARCH ARTICLE}\\
\vspace*{0.5pt}
\\
\includegraphics[align=c,width=0.5cm]{OAlogoblue.png} \space \large\textbf{\color{pciblue}Open Access}\\
\\
\includegraphics[align=c,width=0.5cm]{o_peerreview.png} \space \large\textbf{\color{pciblue}Open Peer-Review}\\
\\
\includegraphics[align=c,width=0.5cm]{o_data3.png} \space \large\textbf{\color{pciblue}Open Data}\\
\\
\includegraphics[align=c,width=0.5cm]{o_script3.png} \space \large\textbf{\color{pciblue}Open Code}\\
\\
\\
\\
\\
\raggedright
%\vspace*{3.25cm}
\scriptsize\textbf{Cite as:}\space
\citeas\\
\vspace*{0.5cm}
\textbf{Posted:} \datepub\\
\vspace*{0.5cm}
\textbf{Recommender:}\\
\recommender\\
\vspace*{0.5cm}
\textbf{Reviewers:}\\
\reviewers\\
\vspace*{0.5cm}
\textbf{Correspondence:}\\
\href{mailto:\email}{\email}\\


}
{\Huge
\fontseries{sb}\selectfont{\preprinttitle}}
\end{flushleft}
\vspace*{0.25cm}
\begin{flushleft}
%\marginpar{


%\marginnote{
%\raggedright
%\vspace*{3.25cm}
%\scriptsize\textbf{Cite as:}\space
%\fullcite{preprint}\\
%\vspace*{0.5cm}
%\textbf{Published:} \datepub\\
%\vspace*{0.5cm}
%\textbf{Recommender:}\\
%\recommender\\
%\vspace*{0.5cm}
%\textbf{Reviewers:}\\
%\reviewers\\
%\vspace*{0.5cm}
%\textbf{Correspondence:}\\
%\href{mailto:\email}{\email}\\
%\vspace*{0.5cm} 
%\vspace*{3cm}
%\vspace*{0.2cm}
%}[0.8cm]


\Large
\listauthors
\end{flushleft}
\bigskip
{\raggedright
\listinstitutions}
% Recommended preprint box
\begin{flushleft}
%\noindent
\fcolorbox{lightgray}{lightgray}{
\parbox{\textwidth - 2\fboxsep}{
\centering\large{\fontseries{sb}\selectfont{This article has been peer-reviewed and recommended by\\
\emph{\PCI}}}\\
%\raggedright\large{\fontseries{sb}\selectfont{An article peer-reviewed and recommended by \emph{\PCI}, edited by \recommender \space on the basis of the reviews by \reviewers \space (DOI: \DOIrecommendationlink)}}\\
%\small \fullcite{preprint}
}}
\end{flushleft}
\vspace*{0.5cm}
\fcolorbox{pciblue}{pciblue}{
\parbox{\textwidth - 2\fboxsep}{
\vspace{0.25cm}
\textbf{\large{\textsc{Abstract}}}\\
\preprintabstract\\

\footnotesize{\textbf{\emph{Keywords: }}\preprintkeywords}
\vspace{0.25cm}}
}
}




